Agentic Design Space Exploration for Joint Hardware Configuration Selection and Mapping of AI Inference Workloads on Heterogeneous Edge SoCs

Modern edge Systems-on-Chip (SoCs) integrate heterogeneous processing units (PUs) such as CPUs, GPUs, and NPUs, each with distinct performance and energy characteristics. Deploying AI inference workloads on them under real-time latency and energy constraints requires jointly mapping workloads to PUs and configuring each PU (e.g., selecting the number of active cores and the operating frequency). This joint space grows combinatorially, making exhaustive search infeasible. Most prior work on design space exploration (DSE) applies black-box optimization (BBO) such as evolutionary search, where each evaluation returns only aggregate metrics such as latency and energy. Recent LLM-guided DSE relies on the same sparse feedback. We observe that this limits its efficiency: it offers no insight into the design space or the reasons a design choice performs the way it does, and it leaves the reasoning abilities of LLMs largely unused. We present TraceDSE, an agentic DSE flow that performs joint workload mapping and PU configuration selection for AI inference on heterogeneous SoCs. TraceDSE is an iterative proposer-critic loop driven by richer feedback in the form of system execution traces. The LLM proposer agent generates candidate mappings and PU configurations for hardware evaluation. The LLM critic agent, equipped with programmatic trace-analysis tools, analyzes the traces to identify bottlenecks and suggest targeted refinements. This loop yields deeper insight into each design point, higher-quality decisions, and a more effective search. Across four AI inference workloads (models of varying complexity and a multi-model pipeline) on an Intel Meteor Lake SoC, TraceDSE consistently outperforms two state-of-the-art BBO tools, improving Pareto frontier hypervolume by up to 35% over NSGA-II and up to 68% over Bayesian optimization, while requiring ~6-9x fewer hardware evaluations.

==> figures/panel_a.tex <==
% Terminal fragment of the HRNet DAG, vertical, schematic upper layers elided with dashes.
\begin{tikzpicture}[x=1pt,y=0.78pt,
  blk/.style={draw=black!70, rounded corners=1pt, fill=blue!30!gray!40, minimum width=14pt, minimum height=7pt, inner sep=0pt},
  term/.style={draw=black, rounded corners=1.5pt, fill=orange!15, font=\scriptsize\ttfamily, inner sep=2.2pt, minimum width=34pt},
  sink/.style={draw=gray!70, rounded corners=2pt, fill=gray!15, align=center, font=\scriptsize, inner sep=2.5pt},
  e/.style={black!60, thin}]
\node[blk] (r) at (80,118) {};
\foreach \i/\x in {1/44,2/62,3/80,4/98,5/116}{\node[blk] (a\i) at (\x,102) {};}
\foreach \i/\x in {1/53,2/80,3/107}{\node[blk] (b\i) at (\x,86) {};}
\foreach \i in {1,...,5}{\draw[e] (r.south) -- (a\i.north);}
\draw[e] (a1.south) -- (b1.north);\draw[e] (a2.south) -- (b1.north);\draw[e] (a2.south) -- (b2.north);
\draw[e] (a3.south) -- (b2.north);\draw[e] (a4.south) -- (b2.north);\draw[e] (a4.south) -- (b3.north);
\draw[e] (a5.south) -- (b3.north);\draw[e] (a1.south) -- (b2.north);\draw[e] (a5.south) -- (b2.north);
\node[term] (t94) at (22,52) {hrnet\_94};
\node[term] (t95) at (61,52) {hrnet\_95};
\node[term] (t96) at (100,52) {hrnet\_96};
\node[term] (t97) at (139,52) {hrnet\_97};
\foreach \t/\s in {t94/b1,t95/b1,t96/b2,t97/b3}{\draw[e, dashed, shorten >=1pt] (\s.south) -- (\t.north);}
\node[font=\scriptsize, gray!40!black] at (80,71) {$\cdots$};
\node[sink] (O) at (80,16) {final output};
\foreach \t in {t94,t95,t96,t97}{\draw[e, ->, >=stealth] (\t.south) -- (O.north);}
\node[align=left, font=\tiny, anchor=north west, text width=62pt] at (168,116)
  {\texttt{hrnet\_94--97}: DAG sinks with the largest per-node latencies (41--70\,ms each)};
\node[align=left, font=\tiny, anchor=north west, text width=62pt] at (168,74)
  {no edges among the four sinks $\Rightarrow$ they can run concurrently on different PUs};
\end{tikzpicture}


==> figures/panel_b.tex <==
% REQUIRES: \usetikzlibrary{patterns,patterns.meta,arrows.meta}
\begin{tikzpicture}[x=1.02pt,y=1pt,line cap=round,line join=round]
% group titles
\node[anchor=south west,font=\scriptsize\bfseries,text width=212.2pt,align=left,inner sep=0pt] at (148.00,90.00) {Candidate X (hrnet\_94$\rightarrow$NPU): 351.6 ms / 8.56 J --- dominated};
\node[anchor=south west,font=\scriptsize\bfseries,text width=212.2pt,align=left,inner sep=0pt] at (148.00,29.50) {Candidate Y (hrnet\_94$\rightarrow$GPU): 297.5 ms / 8.15 J --- new Pareto};
% lane labels
\node[font=\scriptsize,anchor=east,inner sep=0pt] at (146.00,83.00) {GPU};
\node[font=\scriptsize,anchor=east,inner sep=0pt] at (146.00,72.50) {NPU};
\node[font=\scriptsize,anchor=east,inner sep=0pt] at (146.00,22.50) {GPU};
\node[font=\scriptsize,anchor=east,inner sep=0pt] at (146.00,12.00) {NPU};
% candidate 1 bars
\fill[blue!22] (148.00,79.00) rectangle (148.90,87.00);
\fill[orange!27] (148.60,68.50) rectangle (151.20,76.50);
\fill[blue!22] (148.90,79.00) rectangle (150.90,87.00);
\fill[blue!22] (151.30,79.00) rectangle (152.40,87.00);
\fill[blue!22] (152.50,79.00) rectangle (154.30,87.00);
\fill[orange!27] (154.10,68.50) rectangle (157.40,76.50);
\fill[blue!22] (154.30,79.00) rectangle (155.30,87.00);
\fill[blue!22] (155.30,79.00) rectangle (156.00,87.00);
\fill[blue!22] (156.00,79.00) rectangle (157.10,87.00);
\fill[blue!22] (157.60,79.00) rectangle (158.80,87.00);
\fill[orange!27] (158.10,68.50) rectangle (160.50,76.50);
\fill[blue!22] (160.60,79.00) rectangle (161.90,87.00);
\fill[orange!27] (161.50,68.50) rectangle (164.00,76.50);
\fill[blue!22] (162.00,79.00) rectangle (162.60,87.00);
\fill[blue!22] (164.20,79.00) rectangle (165.40,87.00);
\fill[blue!22] (165.40,79.00) rectangle (166.20,87.00);
\fill[blue!22] (166.20,79.00) rectangle (166.90,87.00);
\fill[orange!27] (166.80,68.50) rectangle (171.30,76.50);
\fill[blue!22] (171.50,79.00) rectangle (173.30,87.00);
\fill[blue!22] (173.40,79.00) rectangle (174.90,87.00);
\fill[orange!55] (174.20,68.50) rectangle (237.70,76.50);
\draw[draw=red, line width=0.7pt] (174.20,68.50) rectangle (237.70,76.50);
\node[font=\tiny,text=black,inner sep=0pt] at (205.95,72.50) {h94 63.4};
\fill[blue!22] (175.00,79.00) rectangle (176.10,87.00);
\fill[blue!22] (176.10,79.00) rectangle (177.50,87.00);
\fill[blue!22] (177.60,79.00) rectangle (178.10,87.00);
\fill[blue!22] (178.10,79.00) rectangle (179.10,87.00);
\fill[blue!50] (179.80,79.00) rectangle (233.60,87.00);
\draw[draw=black, line width=0.4pt] (179.80,79.00) rectangle (233.60,87.00);
\node[font=\tiny,text=black,inner sep=0pt] at (206.70,83.00) {h96 53.9};
\fill[orange!55] (238.90,68.50) rectangle (291.10,76.50);
\draw[draw=black, line width=0.4pt] (238.90,68.50) rectangle (291.10,76.50);
\node[font=\tiny,text=black,inner sep=0pt] at (265.00,72.50) {h95 52.3};
\fill[orange!55] (291.70,68.50) rectangle (350.90,76.50);
\draw[draw=black, line width=0.4pt] (291.70,68.50) rectangle (350.90,76.50);
\node[font=\tiny,text=black,inner sep=0pt] at (321.30,72.50) {h97 59.2};
% candidate 5 bars
\fill[orange!27] (148.00,8.00) rectangle (152.80,16.00);
\fill[blue!22] (148.00,18.50) rectangle (148.80,26.50);
\fill[blue!22] (148.90,18.50) rectangle (149.90,26.50);
\fill[blue!22] (152.90,18.50) rectangle (154.40,26.50);
\fill[blue!22] (154.40,18.50) rectangle (156.10,26.50);
\fill[orange!27] (155.40,8.00) rectangle (160.40,16.00);
\fill[blue!22] (156.10,18.50) rectangle (157.60,26.50);
\fill[blue!22] (157.60,18.50) rectangle (158.30,26.50);
\fill[blue!22] (158.40,18.50) rectangle (159.00,26.50);
\fill[blue!22] (160.60,18.50) rectangle (162.00,26.50);
\fill[orange!27] (161.20,8.00) rectangle (163.80,16.00);
\fill[blue!22] (163.90,18.50) rectangle (164.60,26.50);
\fill[orange!27] (164.20,8.00) rectangle (166.40,16.00);
\fill[blue!22] (164.70,18.50) rectangle (166.20,26.50);
\fill[blue!22] (166.50,18.50) rectangle (167.20,26.50);
\fill[blue!22] (167.20,18.50) rectangle (168.70,26.50);
\fill[orange!27] (167.70,8.00) rectangle (170.80,16.00);
\fill[blue!22] (170.90,18.50) rectangle (171.90,26.50);
\fill[blue!22] (172.00,18.50) rectangle (172.90,26.50);
\fill[orange!55] (172.30,8.00) rectangle (238.20,16.00);
\draw[draw=black, line width=0.4pt] (172.30,8.00) rectangle (238.20,16.00);
\node[font=\tiny,text=black,inner sep=0pt] at (205.25,12.00) {h95 65.9};
\fill[blue!22] (172.90,18.50) rectangle (174.30,26.50);
\fill[blue!22] (174.40,18.50) rectangle (175.10,26.50);
\fill[blue!50] (176.10,18.50) rectangle (229.90,26.50);
\draw[draw=black, line width=0.4pt] (176.10,18.50) rectangle (229.90,26.50);
\node[font=\tiny,text=black,inner sep=0pt] at (203.00,22.50) {h96 53.7};
\fill[blue!22] (230.00,18.50) rectangle (232.60,26.50);
\fill[blue!22] (232.70,18.50) rectangle (233.80,26.50);
\fill[blue!22] (233.80,18.50) rectangle (238.80,26.50);
\fill[orange!55] (238.70,8.00) rectangle (297.10,16.00);
\draw[draw=black, line width=0.4pt] (238.70,8.00) rectangle (297.10,16.00);
\node[font=\tiny,text=black,inner sep=0pt] at (267.90,12.00) {h97 58.4};
\fill[blue!50] (241.00,18.50) rectangle (288.90,26.50);
\draw[draw=red, line width=0.7pt] (241.00,18.50) rectangle (288.90,26.50);
\node[font=\tiny,text=black,inner sep=0pt] at (264.95,22.50) {h94 47.9};
% candidate 1 GPU idle region (hatched)
\draw[pattern=north east lines,pattern color=gray!50] (233.60,79.00) rectangle (350.90,87.00);
\node[font=\tiny,text=red,fill=white,fill opacity=0.85,text opacity=1,inner sep=1pt] at (268.00,83.00) {GPU idle 117 ms};
% makespan lines
\draw[dashed,black!70] (350.90,0.00) -- (350.90,27.80);
\draw[dashed,black!70] (350.90,39.20) -- (350.90,87.00);
\node[font=\tiny,anchor=east,inner sep=1pt,fill=white] at (350.90,4.00) {351.6 ms};
\draw[dashed,black!70] (297.10,0.00) -- (297.10,27.80);
\draw[dashed,black!70] (297.10,39.20) -- (297.10,87.00);
\node[font=\tiny,anchor=east,inner sep=1pt,fill=white] at (297.10,4.00) {297.5 ms};
% delta annotation
\draw[{Stealth[length=3pt]}-{Stealth[length=3pt]}] (297.10,56.00) -- (350.90,56.00);
\node[font=\tiny,anchor=south,inner sep=1pt,fill=white] at (324.00,57.20) {$\Delta$ 54.1 ms ($-$15.4\%)};
% time axis
\draw[black] (148.00,0.00) -- (356.00,0.00);
\draw (150.00,0.00) -- (150.00,-2.00);
\node[font=\tiny,anchor=north,inner sep=1pt] at (150.00,-2.00) {150};
\draw (200.00,0.00) -- (200.00,-2.00);
\node[font=\tiny,anchor=north,inner sep=1pt] at (200.00,-2.00) {200};
\draw (250.00,0.00) -- (250.00,-2.00);
\node[font=\tiny,anchor=north,inner sep=1pt] at (250.00,-2.00) {250};
\draw (300.00,0.00) -- (300.00,-2.00);
\node[font=\tiny,anchor=north,inner sep=1pt] at (300.00,-2.00) {300};
\draw (350.00,0.00) -- (350.00,-2.00);
\node[font=\tiny,anchor=north,inner sep=1pt] at (350.00,-2.00) {350};
\node[font=\tiny,anchor=north east,inner sep=1pt] at (144.00,-2.00) {time (ms)};
\end{tikzpicture}


==> figures/panel_c.tex <==
% REQUIRES: \usepackage{pgfplots} \pgfplotsset{compat=1.18}
% Milestone-labelled trajectory; no connector arrows.
\begin{tikzpicture}
\begin{axis}[name=ax1, width=167pt, xmin=261, xmax=366, xtick={280,300,320,340,360},
  ylabel={Energy (J)}, ylabel style={font=\scriptsize,yshift=-3pt}, ytick={8,9,10,11,12}, height=112pt, scale only axis, ymin=7.40, ymax=12.40, tick label style={font=\tiny}, axis line style={gray!60}, major tick style={gray!60}, tick align=outside, clip=true]
\addplot[gray!70, dashed, semithick, mark=square, mark size=1.3pt, mark options={solid, draw=gray!70, fill=white}] coordinates {(285.2,9.19) (287.3,9.07) (287.7,8.36) (299.3,8.14) (307.2,8.11)};
\addplot[gray!70, densely dotted, semithick, mark=triangle, mark size=1.5pt, mark options={solid, draw=gray!70, fill=white}] coordinates {(282.7,12.08) (285.5,9.86) (291.0,8.73)};
\node[font=\tiny, text=gray!30!black, anchor=west, inner sep=1.5pt] at (axis cs:305.0,8.34) {NSGA-II front};
\node[font=\tiny, text=gray!30!black, anchor=west, align=right, inner sep=1.5pt] at (axis cs:264.0,11.82) {Bayesian opt.\\ front};
\addplot[black!85, thick, mark=star, mark size=3.2pt, mark options={color=black}] coordinates {(281.2,9.82) (285.4,8.31) (297.5,8.15)};
\node[font=\tiny, anchor=east, align=right, inner sep=1.5pt, fill=white] at (axis cs:282.80,8.80) {TraceDSE\\ front};
\addplot[only marks, mark=star, mark size=3.2pt, mark options={color=black}] coordinates {(307.20,11.17)};
\addplot[only marks, mark=star, mark size=3.2pt, mark options={color=black}] coordinates {(351.60,8.56)};
\node[font=\tiny, anchor=west, align=left, inner sep=1.5pt, fill=white] at (axis cs:262.30,9.94) {Iter.~1--2:\\ \texttt{h94}$\to$CPU\\ (8/16 cores)};
\node[font=\tiny, anchor=west, inner sep=1.5pt, fill=white] at (axis cs:310.00,11.17) {Iter.~7: \texttt{h94}$\to$CPU, 16 cores (dominated)};
\node[font=\tiny, anchor=north east, align=center, inner sep=1.5pt] at (axis cs:290.60,8.32) {Iter.~6:\\ \texttt{h94},\texttt{h95}$\to$GPU;\\ \texttt{h96},\texttt{h97}$\to$NPU};
\node[font=\tiny, anchor=north west, align=left, inner sep=1.5pt, fill=white] at (axis cs:296.20,8.0) {Iter.~8\\ Cand.~Y: \texttt{h94}$\to$GPU};
\node[font=\tiny, anchor=south east, inner sep=1.5pt, fill=white] at (axis cs:364.00,8.70) {Iter.~8 Cand.~X: \texttt{h94}$\to$NPU};
\node[font=\tiny, text=gray!25!black, anchor=north east, align=right, inner sep=2pt, fill=white] at (axis cs:364.0,12.35)
  {hardware evaluations\\ TraceDSE 94 \textbf{vs.} 723 (NSGA-II), 587 (BO)};
\end{axis}
\begin{axis}[name=ax2, at={(ax1.south east)}, anchor=south west, xshift=10pt,
  width=34pt, xmin=379, xmax=452, xtick={390,430}, yticklabels={,,}, ytick={8,9,10,11,12}, height=112pt, scale only axis, ymin=7.40, ymax=12.40, tick label style={font=\tiny}, axis line style={gray!60}, major tick style={gray!60}, tick align=outside, clip=true]
\addplot[only marks, mark=*, mark size=2.1pt, mark options={fill=gray!55, draw=gray!85}] coordinates {(393.2,11.78) (434.3,8.82)};
\node[font=\tiny, align=center, anchor=north, inner sep=1.5pt, fill=white] at (axis cs:396.0,11.60) {Iter.~0\\all-GPU};
\node[font=\tiny, align=center, anchor=north, inner sep=1.5pt, fill=white] at (axis cs:430.0,8.64) {Iter.~0\\all-NPU};
\end{axis}
\node[font=\small, text=gray!55!black, fill=white, inner sep=0.5pt] at ([xshift=5.5pt,yshift=1.5pt]ax1.south east) {$\cdots$};
\node[font=\scriptsize] at ([xshift=-46pt,yshift=-17pt]ax1.south east) {Latency (ms)};
\end{tikzpicture}


==> figures/panel_dag.tex <==
% Terminal fragment of the HRNet DAG, vertical, schematic upper layers elided with dashes.
\begin{tikzpicture}[x=1pt,y=0.78pt,
  blk/.style={draw=black!70, rounded corners=1pt, fill=blue!30!gray!40, minimum width=14pt, minimum height=7pt, inner sep=0pt},
  term/.style={draw=black, rounded corners=1.5pt, fill=orange!15, font=\scriptsize\ttfamily, inner sep=2.2pt, minimum width=34pt},
  sink/.style={draw=gray!70, rounded corners=2pt, fill=gray!15, align=center, font=\scriptsize, inner sep=2.5pt},
  e/.style={black!60, thin}]
\node[blk] (r) at (80,118) {};
\foreach \i/\x in {1/44,2/62,3/80,4/98,5/116}{\node[blk] (a\i) at (\x,102) {};}
\foreach \i/\x in {1/53,2/80,3/107}{\node[blk] (b\i) at (\x,86) {};}
\foreach \i in {1,...,5}{\draw[e] (r.south) -- (a\i.north);}
\draw[e] (a1.south) -- (b1.north);\draw[e] (a2.south) -- (b1.north);\draw[e] (a2.south) -- (b2.north);
\draw[e] (a3.south) -- (b2.north);\draw[e] (a4.south) -- (b2.north);\draw[e] (a4.south) -- (b3.north);
\draw[e] (a5.south) -- (b3.north);\draw[e] (a1.south) -- (b2.north);\draw[e] (a5.south) -- (b2.north);
\node[term] (t94) at (22,52) {hrnet\_94};
\node[term] (t95) at (61,52) {hrnet\_95};
\node[term] (t96) at (100,52) {hrnet\_96};
\node[term] (t97) at (139,52) {hrnet\_97};
\foreach \t/\s in {t94/b1,t95/b1,t96/b2,t97/b3}{\draw[e, dashed, shorten >=1pt] (\s.south) -- (\t.north);}
\node[font=\scriptsize, gray!40!black] at (80,71) {$\cdots$};
\node[sink] (O) at (80,16) {final output};
\foreach \t in {t94,t95,t96,t97}{\draw[e, ->, >=stealth] (\t.south) -- (O.north);}
\node[align=left, font=\tiny, anchor=north west, text width=62pt] at (168,116)
  {\texttt{hrnet\_94--97}: DAG sinks with the largest per-node latencies (41--70\,ms each)};
\node[align=left, font=\tiny, anchor=north west, text width=62pt] at (168,74)
  {no edges among the four sinks $\Rightarrow$ they can run concurrently on different PUs};
\end{tikzpicture}


==> figures/src/preamble_acm.tex <==
\usepackage[T1]{fontenc}
\usepackage[tt=false, type1=true]{libertine}
\usepackage[varqu]{zi4}
\usepackage[libertine]{newtxmath}


==> tables/seed_variance.tex <==
%%% SEED VARIANCE TABLE %%%
\begin{table}[t]
\centering\small 
\setlength{\tabcolsep}{4pt}
\caption{Five independent TraceDSE runs on ImageBind
(Gemini 3.1 Pro Preview, temperature = 1). All
variance arises from LLM sampling nondeterminism.}
\label{tab:seed_variance}
\begin{tabular}{lrrr}
\toprule
Run & $\widetilde{HV}$ & Tokens (in/out) & Cost (\$) \\
\midrule
1 & 0.758 & 737K / 55K & 4.52 \\
2 & 0.745 & 625K / 45K & 3.82 \\
3 & 0.744 & 748K / 77K & 4.90 \\
4 & 0.764 & 820K / 65K & 5.33 \\
5 & 0.747 & 612K / 45K & 3.75 \\
\midrule
Mean $\pm$ std & 0.752 $\pm$ 0.009
    & 708K $\pm$ 88K / 57K $\pm$ 14K
    & 4.46 $\pm$ 0.65 \\
\bottomrule
\end{tabular}
\end{table}

